Walking on a Graph with a Magnifying Glass: Stratified Sampling via Weighted Random Walks

Our objective is to sample the node set of a large unknown graph via crawling, to accurately estimate a given metric of interest. We design a random walk on an appropriately defined weighted graph that achieves high efficiency by preferentially crawling those nodes and edges that convey greater information regarding the target metric. Our approach begins by employing the theory of stratification to find optimal node weights, for a given estimation problem, under an independence sampler. While optimal under independence sampling, these weights may be impractical under graph crawling due to constraints arising from the structure of the graph. Therefore, the edge weights for our random walk should be chosen so as to lead to an equilibrium distribution that strikes a balance between approximating the optimal weights under an independence sampler and achieving fast convergence. We propose a heuristic approach (stratified weighted random walk, or S-WRW) that achieves this goal, while using only limited information about the graph structure and the node properties. We evaluate our technique in simulation, and experimentally, by collecting a sample of Facebook college users. We show that S-WRW requires 13-15 times fewer samples than the simple re-weighted random walk (RW) to achieve the same estimation accuracy for a range of metrics.

==> abstract.tex <==

\begin{abstract}
Our objective is to sample the node set of a large unknown graph via crawling, to accurately estimate a given metric of interest.
We design a weighted random walk (WRW) algorithm that achieves high efficiency by preferentially crawling those nodes and edges that convey greater information regarding the target metric. Our approach begins by employing the theory of stratification and importance sampling to find optimal node weights, for a given estimation problem, under an independence sampler. While optimal under independence sampling, these weights may be impractical or even unachievable via graph crawling, due to constraints arising from the structure of the graph. Therefore, the weights of WRW should be chosen so as to lead to an equilibrium distribution that strikes a balance between approximating the optimal weights under an independence sampler and achieving fast
convergence. We propose an approach (stratified WRW, or S-WRW) that achieves this goal, while using only limited information about the graph structure and the node properties. We evaluate our technique in simulation, and experimentally, by applying it to infer the ``college friendship graph'' of Facebook. 
We show that S-WRW requires 13-15 times fewer samples than the simple re-weighted random walk to achieve the same estimation accuracy for a range of metrics.



\begin{comment}
%achieves high estimation accuracy with a small sample size (compared to a simple random walk) and limited local information.
%To achieve this goal, first, we build on the theory of \blue{stratified} sampling to find the optimal node weights under an independent node sampler.


%to achieve high efficiency by crawling those nodes and edges  that contribute more to estimation accuracy, by taking into account both the graph structure and the node \blue{properties}.

%The  main challenge lies in choosing the edge weights so as to achieve high accuracy with a small sample size and limited local information.  To achieve this goal, first, we build on the theory of \blue{stratified} sampling to find the optimal node weights under an independent node sampler. However, when node sampling is performed via crawling on the graph, the structure of the graph poses the following challenges: (i) it affects the \blue{equilibrium} distribution  as well as the convergence rate and (ii) only limited information is available about it. In a second step, we design a a weighted random walk (WRW) that assigns edge weights, taking into account both the optimal node weights determined in the previous step and the challenges imposed by  graph crawling. We evaluate our approach   in simulation and experimentally (in Facebook) against simple random walk sampling \blue{[only one baseline, right?]} and we show that it significantly \blue{[numbers?]} improves the estimation accuracy.
%\note{What is wrong with "Finally, we apply WRW to Facebook and we estimate the university-to-university friendship graph."? } %% AM: that is has repetition with the reference to Facebook 2 sentences above.
%% What is in the final evaluation section?
% OLD VERSION
%We introduce a weighted random walk (WRW) as an novel technique to sample large graphs through exploration. WRW achieves high efficiency by exploring more intensively nodes or edges that are relevant for the accuracy of our measurement, and by avoiding the less relevant ones. We enforce it by assigning appropriate edge weights in the sampled graph, which is our main challenge. First, we build on the theory of survey sampling to find optimal node weights under an independent node sampler. Next, we confront these idealistic results with the reality of graph exploration (correlations between sampled nodes, potentially slow convergence rate, limited and noisy prior knowledge about the graph). After we discuss solutions that are optimal (in some sense) yet impractical, we propose a heuristic\note{maybe a name for it?} that uses two easy-to-interpret parameters. We evaluate our technique in simulations and through a real-life implementation on Facebook. In both cases, classic methods (such as random walks and metropolized random walks) require several times more samples to achieve the same accuracy. Finally, we apply WRW to estimate, based on Facebook, a university-to-university friendship graph in the US.


We introduce a weighted random walk (WRW) as an novel technique to sample large graphs through exploration. WRW achieves high efficiency by exploring more intensively nodes or edges that are relevant for the accuracy of our measurement,
%(the more relevant the more likely to be visited),
and by avoiding the less relevant ones.
%mention here the three applications? (magnifying glass, better mixing, low-cost edges)
We enforce it by assigning appropriate edge weights in the sampled graph, which is our main challenge. First, we build on the theory of survey sampling to find optimal node weights under an independent node sampler. Next, we confront these idealistic results with the reality of graph exploration (correlations between sampled nodes, potentially slow convergence rate, limited and noisy prior knowledge about the graph). After we discuss solutions that are optimal (in some sense) yet impractical, we propose a heuristic\note{maybe a name for it?} that uses two easy-to-interpret parameters. We evaluate our technique in simulations and through a real-life implementation on Facebook. In both cases, classic methods (such as random walks and metropolized random walks) require several times more samples to achieve the same accuracy.
Finally, we apply WRW to estimate, based on Facebook, a university-to-university friendship graph in the~US.
\end{comment}
\end{abstract}

% % A category with the (minimum) three required fields
\category{C.4}{Performance of Systems}{Measurement techniques}

\terms{Measurement}


\keywords{Graph Sampling, Weighted Random Walk, Stratified Sampling, Online Social Networks.}



%\begin{itemize}
%  \item Probably I can construct a graph where MHRW performs arbitrarily bad. Take a regular graph with N nodes and add one node $w$ connected to all of them (i.e., of degree N). If $w$ is visited, them very different from not visiting it. A variation - add a couple of deg1 nodes to $w$.
%  \item Produce NetworkX code and offer the code + submit to NetworkX
%  \item Give the WRW sample
%  \item For estimation of average node degree it is PPS (Probability Proportional to Sample), which is good! (low variance)
%  \item total length vs unique length (All sample lengths are shown in unique costs, to reflect precisely the sampling cost)
%Even if we know indegree??
%	\item Speak about PPS, importance sampling, etc
% \item Maybe it is possible to set weights ON THE FLY?? - in phases, yes
% \item This could be cool on directed graphs, but tricky!
% \item Is WRW better than UIS??
% \item Maybe replace $u,v$ with $x,y$ for better readibility?
%\end{itemize}


==> edge_weights.tex <==
%\newpage

%\begin{figure}[!ht]
%	\psfrag{s1}[c]{1}
%
%	\psfrag{a}[c]{\small{ \textbf{Measurement objective}}}
%	\psfrag{b}[c]{\parbox[c]{4.6cm}{\centering \small{\textbf{Optimal weights under WIS}\\ $\w^\WIS(v)$ or $\w^\WIS(C)$}}}  %
%	\psfrag{c}[c]{\parbox[c]{4.6cm}{\centering \small{ \textbf{(Potentially) modified weights}\\ $\tilde{\w}^\WIS(v)$ or $\tilde{\w}^\WIS(C)$ }}}
%	\psfrag{d}[c]{\parbox[c]{4.3cm}{\centering \small{ \textbf{Final edge weights} $\w(e)$}}}
%	\psfrag{e}[c]{\parbox[c]{2.3cm}{\centering \small{ Target edge weights $\tilde{\w}(e)$ }}}
%		%\psfrag{e}[l]{\parbox[c]{3.3cm}{\small{ \textbf{Edge weights} $\w(e)$:\\-~$\w'(C)$ approximated\\-~small mixing time\\-~practical}}}
%		
%		\psfrag{A}[l]{\scriptsize Apply results from Sec.~\ref{sec:Node weight setting under WIS}. Requires $\vol(C)$ ???}
%		\psfrag{B}[r]{\scriptsize No change}
%		\psfrag{C}[l]{\parbox[c]{4.9cm}{\scriptsize{Shaping weights $\w(C)$. Requires:\\-fraction $q$ of irrelevant nodes,\\-maximal resolution $\gamma$, and\\-volume $\vol(C)$.}}}
%		\psfrag{D}[l]{\parbox[l]{2.5cm}{\scriptsize{Minimize mixing\\time as in~\cite{Boyd2004_mixing}}}}
%		\psfrag{E}[l]{\scriptsize Requires $\vol(C)$}
%		\psfrag{F}[l]{\scriptsize Resolve conflicts}
%    \includegraphics[width=0.47\textwidth]{figs/diagram}
%\caption{From objective to setting edge weights.}
%\label{fig:diagram}
%\end{figure}



\newpage
\section{Edge weight setting under WRW}\label{Edge weight setting under WRW}

\subsection{Approach Overview and Rationale}\label{sec:approach-overview}
\maciej{This is long (2 pages) and partially overlapping with the next subsection. I would shrink it (and maybe integrate with the description of \heur?) }

In the previous section, we studied the optimal sample allocation under (independent) stratified sampling.
However, independent node sampling is typically impossible in large online graphs, while crawling the graph is
a natural, available exploration primitive.
%, this is a good starting point %, because WIS is, in a sense, an idealized version of WRW.
In this section, we show how to perform a weighted random walk (WRW) which approximates the stratified sampling
of the previous section.

More specifically, we show how to choose the edge weights, taking into account practical issues that arise in graph exploration. Once the  weights are set, we simply perform a weighted random walk as described in Section \ref{sec:walks} and collect samples. Fig.~\ref{fig:diagram} gives an overview of the steps  taken.



\begin{figure}% top is better
	\psfrag{s1}[c]{1}

	\psfrag{a}[c]{Measurement objective}
	\psfrag{b}[c]{Category weights  $\w^\WIS(C)$ optimal under WIS.}
	\psfrag{c}[c]{ Modified category weights $\tilde{\w}^\WIS(C)$ }
	\psfrag{d}[c]{ Final edge weights $\w(u,v)$ in graph $G$}
  \includegraphics[width=0.47\textwidth]{figs/diagram}
\caption{Overview of our approach: from measurement/estimation objective to setting edge weights.}
\label{fig:diagram}
\vspace{-10pt}
\end{figure}



\subsubsection{Step~1: Setting Category Weights} \label{subsec:From stratified to WIS}

%We adopt the stratified sampling technique for the purpose of network sampling.
We start from the measurement objective and we compute the node weights (or equivalently the number of samples per category) as in the previous section. Ideally, we would like to enforce strictly stratified UIS or WIS. However, when we use crawling instead of independence sampling, sampling exactly~$n_i$ nodes from category~$C_i$ is (and no other nodes) is possible only by discarding observations. 
% (since not all graphs have walks visiting each category a fixed number of times).  
It is thus more natural to frame the problem in terms of the probability mass placed on each category in equilibrium, or equivalently the \emph{expected} number of nodes drawn in each category given the total sample size.  This does not change the above UIS/WIS framework, and the above weights apply exactly as before.  
%Likewise, when sampling from a Markov chain, it is clear that our target pmf is attained only in the limit of infinite sample size (as an equilibrium distribution) implying some degree of bias for finite samples.
%We soften this restrictive requirement by setting the weight of every node $v\in C_i$ to:
%\begin{equation} \label{eq:w in From stratified sampling to weighted sampling}
%	\w^\UIS(v) = 1 \qquad \textrm{ and } \qquad \w^\WIS(v) = \frac{n^\opt_i}{|C_i|},
%\end{equation}
%thus making WIS collect~$n_i$ samples in category~$C_i$ in expectation.\blue{[Question to Carter]}
%\footnote{\note{Any comments? CARTER, could you help motivate this `in expectation' transition? Mention that all variances and gains calculated before, hold in expectation, for UIS and WIS. But how to calculate precisely these variances? Technically, what happens if we do not to collect any single sample from a given category? Does variance go to infinity?? (Even if we condition on having at least one sample per category, then the formulas become ugly.)}}
%CTB: No, the estimator variances will not go to infinity.  Remember, Var(z)=E(z^2)-E(z)^2; so long as z^2 is finite, Var(z) will exist.
%CTB: BTW, I commented out the above, b/c you don't need to change the weights, and in fact doing so doesn't accomplish anything that I can see.

%A more serious concern when moving from independence sampling to link-trace sampling is that it may not be possible to attain a given target expectation $n_i^\opt/n$ even in the limit $n\to \infty$.  For instance, if the induced subgraph $G[\mathcal{C}\setminus\{C_\Theta\}]$ is disconnected, then there exists no Markov chain that almost surely both places no mass on the elements of $C_\Theta$ and which places positive masses on all elements of $\mathcal{C}\setminus\{C_\Theta\}$ in the inifinite limit of sampling.  In such situations, we may be forced to compromise by selecting an equilibrium distribution that is less efficient, but attainable.  We discuss this in greater detail below.



Furthermore, we move from the weights of individual nodes to the weights of entire categories. One can think of the problem in two levels of granularity: the original graph $G\eq (V,E)$ and the {\em category graph} $G^C \eq (\mathcal{C}, E^C)$. In~$G^C$, nodes represent categories, and every undirected edge $\{C_1,C_2\}\in E^C$ represents  %there is at least one edge between $C_1$ and $C_2$ in the original graph, \ie:
the corresponding non-empty set of edges $E_{C_1,C_2}\subset E$ in the original graph~$G$, \ie
$$E_{C_1,C_2}\ = \{\{u,v\}\in E:\ u\in C_1 \textrm{ and }  v\in C_2\} \neq \emptyset.$$
%edge $\{C_1,C_2\}$ exists only when $|E_{C_1,C_2}|\geq 1$.
The rationale for moving from the finer granularity of $G$ to the coarser granularity of $G^C$ is twofold.
From a theoretical point of view, categories are exactly the properties of interest in the estimation problems we consider. From a practical point of view, it is relatively easy to obtain or infer information
about categories (\ie the category a node belongs to and the relative size of categories); see Section \ref{subsec:Limited initial information}.

%However, in practice, we cannot really distinguish the nodes to work at this resolution \maciej{TO EXPLAIN}.

% \note{Mention somewhere, that $G$ is assumed to be connected.} %% Athina: Yes in secton 2: hen you say it is also static, indirected and connected.

%\smallskip

%The weight setting problem can be defined at both levels. In $G$, every node $v\in V$ has to meet its target weight~$\w(v)$. In contrast,

   Setting node weights in the category graph $G^C$ requires that every category $C_i\subset V$ meets its target weight $$\w^\WIS(C_i)\ =\ \sum_{v\in C_i}\!\w^\WIS(v)\ =\ n^\opt_i.$$
However, the actual distribution of this aggregated category weight among nodes in~$C_i$ does not matter. By setting $\w(C_i)$,  we control the expected number~$n_i$ of samples from~$C_i$, because $n_i\propto \w(C_i)$.
%
%must have different weights, we can still try to control the (expected) number~$n_i$ of samples to collect from~$C_i$, i.e., at the level of graph~$G^C$. Indeed, $n_i$ is proportional to the weight~$\w(C_i)$ of this category, i.e.,  \note{Is it obvious?}
%$$n_i\ \sim\ \w(C_i)=\sum_{v\in C_i}\w(v).$$
%
Working at this coarse granularity sacrifices performance (\eg we might be able to achieve faster mixing by considering the connectivity within each category) for simplicity and practicality (information at fine granularity $G$ is more expensive or impossible to obtain). In the next steps, we focus on setting the edge weights in $G$ based on the coarse-grained information available in $G^C$.



\begin{figure}[t]
		\psfrag{a}[l]{$w_1$}
		\psfrag{b}[c]{$w_2$}
		\psfrag{A}[l]{\textbf{(a)}}
		\psfrag{B}[l]{\textbf{(b)}}
		\psfrag{X}[l]{\parbox[c]{3.6cm}{\small{WIS:\hspace{0.22cm} $\w_1\!>\!0,\ \w_2\eq0$\\WRW: $\w_1\eq 0,\ \w_2\!>\!0$}}}  %
		\psfrag{Y}[l]{\parbox[c]{3.6cm}{\small{WIS:\hspace{0.23cm} $\w_1 = 190\, \w_2$\\WRW: $\w_1 \cong 25\, \w_2$}}}  %	
    \includegraphics[width=0.46\textwidth]{figs/tiny_example}
\caption{Optimal edge weights: WIS vs WRW.   \maciej{Under what sampling length? And what objective? How did we get these numbers? (simulations)}}
\label{fig:tiny_example}
\vspace{-10pt}
\end{figure}




\subsubsection{Step~2: Modifying Category Weights}\label{sec:step2-general}

A key observation is that the optimal category weights $\w^\WIS(C_i)$ under WIS are not necessarily optimal under WRW. As discussed in the introduction, the target equilibrium distribution  $\pi^\WRW$ under WRW
should be chosen so that it is close to $\pi^\WIS$ but also achieves fast mixing.

Let us re-visit this intuition using the toy example in Fig.~\ref{fig:tiny_example}(a). %Due to symmetry,
We distinguish between two types of edges and their corresponding weights $\w_1$ and $\w_2$.
 If we are interested in measuring the average value of a property over the dark nodes only, then the optimal weights under WIS are $\w_1>0$ and $\w_2=0$: WIS samples each green node with the same probability and never samples the white one. However, under WRW with these weights, the dark nodes are disconnected into two components and WRW does not converge. One can show that under WRW, the optimal weights are $\w_1=0$ and $\w_2>0$: half of the samples are due to visits in the white (irrelevant) node.

 Therefore, when sampling via WRW, we may have to move away from $\pi^\WIS(C_i)$ to another target equilibrium distribution $\tilde{\pi}^\WIS(C_i)\neq \pi^\WIS(C_i)$, which trades the optimality of WIS weights for faster mixing
 %\footnote{Interestingly, the edge weights that achieve fastest mixing do not lead to the optimal solution either. Indeed, minimizing the second eigenvalue of WRW transition matrix~\cite{Boyd2004_mixing} results in weights $2\, \w_1\eq \w_2$.} %%% not now.
and higher overall quality of estimation. Equivalently, in the second step of our approach, we move from
$\w^\WIS(C_i)$ to $\tilde{\w}^\WIS(C_i)\neq \w^\WIS(C_i)$.
%We illustrate this transition as Step~2 in the diagram in Fig.~\ref{fig:diagram}.


%If in graph $v_1-v_2-v_3$ we are interested in measuring $v_1$ and $v_3$ only, then WIS would clearly set $w(v_2)=0$. For WRW, however, this means a disconnected graph and no convergence at all, which is not at all optimal. Therefore, to improve the estimation quality, we sometimes have to trade the optimality of $\Pi^\WIS$ for a better convergence of $WRW$.

%\note{We can probably capture that by calculating the expected time WRW will stay at the edges of community $C$. This time is proportional to $w(C) / w(\textrm{closest neighborhood of }C)$. If this time is larger than $n\cdot w(C)/\sum_i w(C_i)$ , then it is definitely not good. Hopefully, we can formalize it better.}

\textbf{Optimal solution.}
 The optimal $\tilde{\w}^\WIS(C_i)$ should minimize the total estimation error, which consists of two parts:
the error due to the sampling distribution being different from  $\pi^\WIS(C_i)$, and the error due
to lack of convergence for finite number of samples. We have obtained numerical solutions in toy examples.
However, solving the general optimization problem is not only difficult but also requires the full knowledge of the graph and potentially the values $x(v)$ carried by the nodes; this information is not available in practice. 
The optimization of $\tilde{\w}^\WIS(C_i)$ is out of the scope of this paper.\footnote{It is worth noting that even optimizing only for the mixing time, which is part
of the problem, is non-trivial. A solution is only known assuming complete knowledge of the graph \cite{Boyd2004_mixing}.}

Instead, we provide intuition for modifying the category node weights so as to trade-off some of the optimality of WIS for faster mixing. We follow these guidelines later in the design of our practical solution \heur.

\textbf{Guideline 1: occasionally visit irrelevant nodes.}
We have seen in the examples in Fig. 1 and Fig.~\ref{fig:tiny_example} that WRW may benefit from allocating small
weight $\w(C_\ominus)\!>\!0$ to category $C_\ominus$ that is not directly relevant to our estimation. The intuition is that
irrelevant nodes may not contribute to estimation but may be needed for connectivity or fast mixing.

%WIS has a direct access to all the nodes, regardless of graph topology. In contrast, WRW is an exploration technique, which, at some current node, has the access to its neighbors only. We have to remember about it, especially when measuring only a particular category $C\subset V$ of nodes (Sec.~\ref{subsec:Measuring only particular category of nodes}). Under WIS, we can simply set to 0 all the weights of (irrelevant) nodes in~$V\m C$. However, under WRW, zeroing these nodes~$V\m C$ (by setting to 0 all weights of edges $E(V\m C)$ incident on them) is not a good practice in general. Indeed, if~$C$ does not induce a connected subgraph of~$G$ (see Fig.~\ref{fig:illustration_magnifying_glass} for an example), we will not be able to reach all nodes in~$C$ and thus WRW will never converge. Instead, we should allow WRW to benefit from all edges in $G$, by setting the weights of edges $E(V\m C)$ to positive yet small values.



%How small these weights should be? Below we provide some practical hints:
%\begin{itemize}
%	\item WRW should visit mostly (but not exclusively) the relevant nodes. Therefore, set the weights such that, say,  $0.01<\w(C_\ominus)/\w(tot)<0.50$. As a result, WRW will visit nodes in $V\m C$ only in 1\% to 10\% of iterations.
%	\item Imagine WRW is arriving from $u\in C$ at node $v\in V\m C$. If all the neighbors of $v$ (except for $u$) are also in $V\m C$, we would like to have a non-negligible probability of following one of them (i.e., returning to $u$ should not be a far dominating option). For this reason, $\w(C,V\m C)$ should be comparable with $\bar{k}\cdot \w(V\m C, V\m C)$, where $\bar{k}$ is the average node degree in $G$.
%	\item If we do expect that $C$ forms disconnected components in $G$, we can also think of typical distances between these components ans set $\w(V\m C, V\m C)$ high enough to traverse them.
%\end{itemize}


\textbf{Guideline 2: avoid ``black holes''.}
  Every optical system has a fundamental magnification limit due to diffraction %~\cite{Wikipedia_difraction_limited_system} 
  and our ``graph magnifying glass'' is no exception. Consider the toy graph in Fig.~\ref{fig:tiny_example}(b): it consists of a clique of 20 red nodes with edge weights $w_2$, and a loop with two green nodes with edge weights $w_1$. In Section~\ref{subsec: Relative sizes of node categories}, we saw that WIS optimally estimates the relative sizes for equal expected number of samples from the two categories; this is the case for $w_1\eq 190\,w_2$. However, for such large values of $w_1$, the two green nodes behave as a sink (or a ''black hole'') for a WRW of finite length, thus  increasing the variance of the category size estimation. 
In other words, although WIS suggests over-sampling small categories,  WRW should ``under-over-sample'' very small categories to avoid black holes. Indeed, we found %in simulation 
$w_1\eq 25\,w_2$ to be optimal for this example.

%we will treat all categories smaller than $\vol(C_{min})$ as equal to $\vol(C_{min})$. The choice of $\vol(C_{min})$ strongly depends on the topology. In our experiments with Facebook we set $\vol(C_{min})$ equal to $1/1000$ of the volume of the biggest category $\vol(C_{max})$. As a rule of thumb, the ratio $\vol(C_{max})/\vol(C_{min})$ should be comparable with the average node degree (say within one order of magnitude).

%There is one more practical reason to introduce $\vol(C_{min})$: In the pilot run (see below), we are likely not to discover some small categories. Without any estimate of their volume, we just set them by default to $\vol(C_{min})$.


%\note{Actually, this is not a big issue in Facebook, so maybe I will skip this and related parts of this paper for the sake of simplicity}
%Another problem is that the optimal node weights calculated for WIS are not necessary optimal under WRW. We presented a good example of that in Fig.~\ref{fig:illustration}B, where WRW performs best for a different weight setting from WIS. The main reason of this phenomenon is that every walk (including WRW) introduces correlations between visited nodes.
%In an extreme case, if a very small and tight community is given very high node weights (optimal under WIS), it will almost become a sink for the WRW. This naturally increases the variance of the estimator of the category size, for example.


%So the optimal weight setting under WRW is probably somewhere in between WIS and RW (i.e., every edge has weight 1).



\subsubsection{Step~3: Setting Edge Weights in G\label{sec:step3-general}}
Once the  node category weights have been fixed to $\tilde{\w}^\WIS(C)$, the next step is to choose the edge weights, in graph $G^C$, and eventually the edge weights in the original graph~$G$ where the crawl is performed.
%

%CTB: Note on below: getting the category weights right is not enough: we must draw each vertex with a probability proportional to its category weight.  Loops aren't enough for that -- you need to assume that G[\mathcal{C}\setminus\{C_\Theta\}] is connected.
\maciej{Rewrite!}
It is always possible to set the edge weights in~$G$ so as to achieve an arbitrary category weight allocation $\w(C)$ in $G^C$, under the assumption that there are self loops in each category $\{C,C\}$ in $G^C$. A proof is provided in Appendix A. The condition about self-loops is mild to satisfy in practice: it only requires that every category $C$ has at least one intra-category edge in $G$.
However, the construction is not unique: there are many  ways to set the edge weights and achieve the same goal.
Given that the node weights (or equivalently the equilibrium distribution $\pi^{WRW}$) are set in the previous step, the best choice of edge weights in this step is the one that minimizes the mixing time.

%\note{Here say a few words about the connection between variance, spectral gap $\delta$, and mixing time. Similarly to Section~1 in \cite{Avrachenkov2010}. Check \cite{AldousBookInPreparation}. Also~\cite{Lovasz93,Boyd2004_mixing,Mohaisen2010}}
%Intuitively, the faster the walk changes the regions in the graph the better.

\textbf{Optimal Solution.}
 In \cite{Boyd2004_mixing}, the fastest mixing Markov Chain that achieves a target equilibrium distribution has been computed exactly using convex optimization, assuming that the entire graph is known.
It is impossible to apply these techniques in $G$, due to the lack of perfect, global information about $G$ in our problem context: if we knew $G$, there would be no need for sampling. Instead, one could apply the technique in \cite{Boyd2004_mixing} to set the weights in $G^C$, after estimating some limited information about $G^C$, as in Appendix B and Section \ref{subsec:Limited initial information}, and then translate them into edge weights in $G$. If the categories $C_1$ and $C_2$ are connected by an edge with weight $\w^C(C_1,C_2)$ in $G^C$, then the weight of every edge in $G$ between $C_1$ and $C_2$ should be $\w(C_1,C_2) = \w^C(C_1,C_2)\, /\, |E_{C_1,C_2}|$. There are two problems with the latter approach: our estimates of $G^C$ may be inaccurate; furthermore,  optimal edge weights in $G^C$ do not necessarily translate into optimal edge weights  in $G$.



\begin{comment}
\subsubsection{Optimal (but impractical) solution}
Theoretically, we can apply the technique from~\cite{Boyd2004_mixing} to maximize the spectral gap of WRW's transition matrix, and, consequently, minimize the mixing time.
However, not surprisingly, this technique, requires the knowledge of the entire graph.
%\subsection{Our idealistic solution at level $G$}
At the level of $G$, this is completely impractical.
%\subsection{Our idealistic solution at level $G^C$}
%Assume also that we want the same number of samples from each category. With all this knowledge, we are able to set the weights of edges $E^C$ optimally (in terms of mixing time) and efficiently. Indeed, we just have to apply the approach in~\cite{Boyd2004_mixing}.

In contrast, we can assume to have some (limited) view of graph~$G^C$. We can feed it to the algorithm~\cite{Boyd2004_mixing} to optimize the mixing time at the level~$G^C$.
%Theoretically, it is easy to translate these results into the weights in the underlying graph~$G$.
Now, if in $G^C$ the categories $C_1$ and $C_2$ are connected by edge with weight $\w^C(C_1,C_2)$, then the weight of every edge in $G$ between $C_1$ and $C_2$ should be $\w(C_1,C_2) = \w^C(C_1,C_2)\, /\, |E(C_1,C_2)|.$
%(If $C_1=C_2$ then we are talking about a self-loop in $G^C$ internal edges in $G$.)


There are two main problems with this approach.
%
First, our estimates of $|E(C_1,C_2)|$ may be very inaccurate, especially for small $C_1$ and $C_2$.
%, we are likely to have $|E(C_1,C_2)|=0$ .
%Indeed, the `pilot' RW (Sec.~\ref{subsec:Limited initial information}) can help us estimate the numbers of internal and external edges for categories, but with a higher variance. Indeed, an internal edge (in contrast to external edges) is discovered only when RW samples at least one of its end-nodes, which may be very rare for smaller categories.
This directly affects the values $\w(C_1,C_2)$ we set.

Second, even given a perfect knowledge of $|E(C_1,C_2)|$, we may often end up having a huge weight $\w(C_1,C_2)$, e.g., for $|E(C_1,C_2)|=1$. Such a heavy weight edge may act as a black hole alone (or more like a `double pulsar' such as PSR~J0737-3039). For this reason, we wish to have more control over the range of weights $\w(C_1,C_2)$.

\end{comment}


\textbf{Guideline 3: prefer inter-category edges.}
%The construction given in Appendix A, when applied in $G$ %Observation~\ref{theorem:edge_weigh_assignment_feasibility}
%achieves the desired target category node weights but may result in high weights on intra-category edges and small weights on inter-category edges. % is fixed to a small value.
There are several possible edge weight assignments that achieve the desired category node weights. High weights on intra-category edges and small weights on inter-category edges result in WRW staying in small categories~$C_{tiny}$ for a long time. 
In order to improve the mixing time, we should do exactly the opposite, \ie  assign relatively high weights to inter-category edges (connecting relevant categories). As a result, WRW will enter $C_{tiny}$ more often, but will stay there for a short time.
This intuition is motivated by Monte Carlo variance reduction techniques such as the use of antithetic variates~\cite{Gentle2003}, which seek to induce negative correlation between consecutive draws so as to reduce the variance of the resulting estimator.







\subsubsection{Operating with Limited Information}\label{subsec:Limited initial information}
%\note{Where should we put it?} % I suggest either inside Step~1 (to motivate moving to $G^C$ level), or in the very front of Sec.~\ref{subsec:heur}}

\textbf{Information needed for setting edge weights (before the crawl).}
 In order to set the edge weights, we need some prior information about the graph $G$, such as: the sizes and volumes of the node categories, their ``tightness'' (\eg measured by the ratio of numbers of internal and external edges), the size and topology of the irrelevant category, the topology of of the category graph $G^C$, etc. The more information we have, the better.
However, before the sampling begins, our knowledge about $G$ is by definition limited or altogether absent; otherwise, there would be no need to sample the graph.
However, it may still be possible to obtain or infer information from other sources. For example, we may know the size of categories (the size of universities in Facebook is publicly available); or we may run a short ``pilot RW'' to get rough estimates of the properties in question. For example, in Appendix~B, we derive an efficient and unbiased estimator of volumes $\vol(C)$ based on a pilot random walk.

\textbf{Information needed about the neighbors (during the crawl).} During WRW, we jump from the current node $v$ to one of the neighbors $u$ with probability $P_{v,u}=\frac{\w(v,u)}{\sum_{u'} \w(v,u') }$. In order to use the right weight $\w(u,v)$, WRW must have some information on these neighbors before visiting them. We require minimal information about the membership of $u$ to category $C(u)$. Fortunately, such information is often available in most online  graphs. For example, when inferring the college friendship graph in Facebook (Section~\ref{subsec:Friendly universities}), we use the college membership information of all~$v$'s neighbors, which, in Facebook, is available at~$v$ together with the friends list. Even when the relevant information is not available directly, we can sometimes infer it from other attributes without actually visiting the node. For example in OSNs, we may exploit the neighbors's name to identify their nationality and follow edges between users with different nationality to reach different parts of the graph and improve mixing time. Even mere node IDs (which are available in every crawlable system) may be exploited. For example, some chunks of ID space are often associated with particular servers, creating a clear correlation between ID and its geographical location.






%\subsection{Our practical solution: \heur}\label{subsec:heur}
%
%%A practical weight setting algorithm should trade between the amount of required input data, its accuracy, and the cost of obtaining it.
%In this section, we introduce our practical heuristic solution - {\em Stratified Weighted Random Walk} or \heur.
%\heur follows the steps and rationale of the general approach in Section \ref{sec:approach-overview} and makes the following specific choices.
%\heur uses as input only the estimates $\lowhat{\vol}(C)$ of the category volumes (see Appendix B). 
%\heur uses two natural and easy-to-interpret parameters, $\tilde{f}_\ominus$ and $\gamma$, in order to achieve approximately  $\w^\WIS(C_i)$.
%
%\subsubsection{Step 1: Setting Category Weights}
%In Sec.~\ref{sec:Node weight setting under WIS}, we calculated, under various scenarios, the optimal (and often equal) WIS category weights~$\w^\WIS(C_i)$. \heur uses these weights as the main guideline. 
%%Given our estimation problem, we set the expected number of samples per category or, equivalently, the category node weight $\w^\WIS(C_i)$.
%%\heur sets the edge weights trying to achieve roughly $\w^\WIS(C_i)$ as described below. 
%
%Usually, there are many edge weight settings in~$G$ that achieve~$\w^\WIS(C_i)$. 
%%We choose to divide the total weight of a category equally across all $\vol(C_i)$  edges that are incident to nodes in~$C_i$ (see Eq.(\ref{eq:volume})), s.t. each edge $e$ has the same weight % $w_e$:
%In our implementation, we observe that~$\vol(C_i)$ counts the number of edges incident on nodes of~$C_i$. Consequently, if for every category~$C_i$ we set in~$G$ the weights of all edges incident on nodes in~$C_i$ to
%\begin{equation}\label{eq:w_e(C_i)}
%%	\w_e(C_i)\ =\ \frac{n^\opt_i}{\vol(C_i)},
%	\w_e(C_i)\ =\ \frac{\w^\WIS(C_i)}{\vol(C_i)}.
%\end{equation}
%then $\w^\WIS(C_i)$ is achieved.\footnote{There exist many other edge weight assignments that lead to $\w^\WIS(C_i)$. \eqn{\ref{eq:w_e(C_i)}} has the advantage of distributing the weights evenly across all~$\vol(C_i)$ edges.}
%This simple observation is central to the \heur heuristic. 
%Indeed, \heur tries to satisfy \eqn{\ref{eq:w_e(C_i)}} with the modifications described below.
%
%
%
%
%\subsubsection{Step~2: Modifying Category Weights}
%
%\textbf{Irrelevant categories.}
%Let us group all (if any) irrelevant categories  into a single irrelevant category $C_\ominus\in \mathcal{C}$. Although $\w^\WIS(C_\ominus)=0$, Guideline 1 in Section \ref{sec:step2-general} suggests that we place some mass on irrelevant nodes to ensure convergence. In \heur, we achieve this goal by replacing $\w^\WIS(C_i)$ with
%%$$
%%\tilde{n}_i^\opt = \left\{
%%	\begin{array}{ll}
%%			n_i^\opt & \textrm{if } C_i \neq C_\ominus\\			
%%			q\cdot n & \textrm{if } C_i = C_\ominus.		
%%		\end{array}	
%%		\right.
%%$$
%\begin{equation}
%\tilde{\w}^\WIS(C_i) = \left\{
%	\begin{array}{ll}
%			\w^\WIS(C_i) & \textrm{if } C_i \neq C_\ominus\\			
%			\tilde{f}_\ominus \cdot \sum_{C\neq C_\ominus} \w^\WIS(C) & \textrm{if } C_i = C_\ominus.		
%		\end{array}	
%		\right.
%\end{equation}
%The parameter $0<\tilde{f}_\ominus\ll 1$ controls the desired fraction of times we visit nodes in $C_\ominus$. The optimal choice of $\tilde{f}_\ominus$ depends on many factors, such as the distribution of relevant and irrelevant nodes on the graph and their absolute numbers. When measuring Facebook in Section~\ref{Applications}, we set~$\tilde{f}_\ominus=1\%$. %and $\tilde{f}_\ominus\rightarrow 0$ if $C_\ominus$ is relatively small.
%
%\textbf{Tiny and unknown categories.}
%Guideline 2 in Section \ref{sec:step2-general} suggests that we should avoid ``black holes''. In \heur, we achieve this goal by replacing $\vol(C_i)$ in \eqn{\ref{eq:w_e(C_i)}} with
%\begin{eqnarray}
%\nonumber \lowtilde{\vol}(C) &=& \max\Big\{\lowhat{\vol}(C),\ \vol_{min}\Big\},\quad \textrm{ where }\\
%\nonumber \vol_{min} &=& \frac{1}{\gamma}\cdot \max_{C\neq C_\ominus}\{\lowhat{\vol}(C)\}
%\end{eqnarray}
%and $\lowhat{\vol}(C)\eq 0$ if $C$ is not covered by our estimate. This allows us to accommodate all unknown categories.
%
%The parameter $\gamma\geq 1$ corresponds to the maximal magnification of our ``graph magnifying glass''. For $\gamma\eq 1$ (and constant~$\w^\WIS(C_i)$), we are back to the simple random walk. For $\gamma\rightarrow\infty$, we may face the problem of ``black holes'' as discussed in Sec.~\ref{sec:step2-general}. We recommend setting $\gamma$ to a value a few times larger than the average node degree $\bar{k}$.
%%\footnote{$\bar{k}$ is often known, or can be easily estimated in the pilot RW}
%In Section~\ref{Applications}, we use roughly $\gamma = 10\cdot \bar{k}$. %\note{motivate this better?}
%%CTB: What about the approximate escape time rationale?
%
%
%
%\subsubsection{Step 3: Setting Edge Weights in $G$} \label{subsec:Resolving Conflicts}
%With the above modifications, our target edge weights defined in Eq.(\ref{eq:w_e(C_i)}) can be rewritten as
%%Similarly to Eq.(\ref{eq:w_e(C_i)}), we distribute the total weight of a category $C_i$ equally across all the $\vol(C_i)$  edges that are incident to nodes in $C_i$:
%%Furthermore, recall that $\vol(C_i)$ counts the number of edges incident on nodes of~$C_i$. Consequently,
%%if for every node category~$C_i$ we set in~$G$ the weights of all edges incident on~$C_i$ to
%\begin{equation}\label{eq:tilde w_e(C_i)}
%	\tilde{\w}_e(C_i)\ =\ \frac{\tilde{\w}^\WIS(C_i)}{\lowtilde{\vol}(C_i)}.
%\end{equation}
%%If such an assignment is possible, then WRW achieves $\tilde{\w}^\WIS(C_i)$.
%%
%We can directly set the weight $\w(u,v)\eq\tilde{\w}_e(C(u))\eq\tilde{\w}_e(C(v))$ of an intra-category edge $\{u,v\}$. However, for every inter-category edge, we usually have ``conflicting'' weights  $\tilde{\w}_e(C(u))\neq \tilde{\w}_e(C(v))$ required at the two ends of the edge. We choose to assign an edge weight  $\tilde{\w}_e$ that is in between these two values $\tilde{\w}_e(C(u))$ and $\tilde{\w}_e(C(v))$.
%We considered several candidate  such assignments.
%We may take the {\em arithmetic} or {\em geometric} mean of the conflicting weights, which we denote by $\w^{arithmetic}(u,v)$ and $\w^{geometric}(u,v)$, respectively. We may also use the {\em maximum} of the two values, $\w^{max}(u,v)$, which should improve mixing according to Guideline 3 in Section \ref{sec:step3-general}. %~\ref{subsec:Better RWR mixing through heavier external links}.
%However, $\w^{max}(u,v)$ alone would also add high weight to irrelevant nodes $C_\ominus$. To avoid this undesired effect, per Guideline 1, we distinguish between the two cases by defining a hybrid solution:
%$$
%        \w^{hybrid}(u,v) = \left\{
%        \begin{array}{ll}
%                        \w^{geometric}(u,v)  & \textrm{if }C_\ominus\in\{C(u),C(v)\}\\
%                        \w^{max}(u,v) &\textrm{otherwise.}
%                \end{array}
%                \right.
%$$
%
%
%
%This hybrid edge assignment was the one we found to work best in practice - see Section \ref{Applications}.
%
%%\begin{equation}
%%	\w^{arithmetic}(u,v) = (\tilde{\w}_e(C(u)) + \tilde{\w}_e(C(v)))/2   \hspace*{6in}
%%\end{equation}
%%
%%\begin{equation}
%%	\w^{geometric}(u,v) = \sqrt{\tilde{\w}_e(C(u))\cdot\tilde{\w}_e(C(v))}   \hspace*{6in}
%%\end{equation}
%%
%%\begin{equation}
%%	\w^{max}(u,v) = \max\left(\tilde{\w}_e(C(u))\cdot\tilde{\w}_e(C(v))\right)   \hspace*{6in}
%%\end{equation}
%%
%%\begin{equation}
%%	\w^{hybrid}(u,v) = \left\{
%%	\begin{array}{ll}
%%			\sqrt{\tilde{\w}_e(C(u))\cdot\tilde{\w}_e(C(v))}  &  \back\back\back\textrm{if }C_\ominus\in\{C(u),C(v)\}\\
%%			& \\
%%			\max\big\{\tilde{\w}_e(C(u)), \tilde{\w}_e(C(v))\big\} &\textrm{otherwise.}
%%		\end{array}	
%%		\right.
%%\end{equation}
%
%
%
%
%
%
%\subsubsection{Information Required and Discussion}
%
%%\begin{comment}
%%\heur sets the edge weights trying to achieve roughly $\w^\WIS(C_i)$ as the main goal.
%%Through two natural and easy-to-interpret parameters, $\tilde{f}_\ominus$ and $\gamma$, we slightly shape $\w^\WIS(C_i)$
%%%%the target distribution
%%to avoid black holes and improve mixing.
%%It corresponds to Step~2 in Fig.~\ref{fig:diagram}. Step~3 under \heur can be decomposed into two substeps. First, we use~\eqn{\ref{eq:tilde w_e(C_i)}} to calculate the desired edge weights in~$G$. Next, we set these values to actual edges and
%%%%The same objectives are taken into account when
%%resolve potential conflicts.
%%\end{comment}
%
%\textbf{Information Required.} The only inputs that \heur needs in order to set the weights before the crawl are the estimates of the category volumes $\lowhat{\vol}(C)$. These are easy and inexpensive to obtain either explicitly or via short pilot runs; see Section \ref{subsec:Limited initial information} and the estimators in Appendix B. The only information that \heur needs during the crawl is the category each neighbor belongs to; see  Section \ref{subsec:Limited initial information}.
%
%
%
%%\noindent The above procedure has the following properties:
%%\begin{itemize}
%%	\item The edge weights of category $C$ are, in general, proportional to $\w'(C)/\vol(C)$, which guarantees that the resulting category weight $\w(C)$ is similar to the desired one $\w'(C)$.
%%	\item The very small categories and the categories not discovered in the pilot RW are all assumed to have volume $\vol_{min}$. This is to avoid the black hole effect (see Sec.~\ref{subsec:Correlations - avoiding the black holes}), and to accommodate unknown categories.
%%	\item Every inter-category edge weight is determined by the smaller (or `weightier') of the two categories. This is to improve mixing, as discussed in Sec.~\ref{subsec:Better RWR mixing through heavier external links}. Note that the larger category $C_{big}$ will receive some heavyweight edges from smaller categories, possibly resulting in $\w(C_{big})>\w'(C_{big})$. This side effect slightly shifts WRW towards RW (where $\w(C)=\vol(C)$ for every $C$), which is conservative.
%%\end{itemize}
%
%\begin{figure*}
%\begin{center}
%		\psfrag{A}[r][]{\textbf{(a)}}
%		\psfrag{B}[r][]{\textbf{(b)}}
%		\psfrag{C}[r][]{\textbf{(c)}}
%		\psfrag{D}[r][]{\textbf{(d)}}
%		\psfrag{E}[r][]{\textbf{(e)}}
%		\psfrag{F}[r][]{\textbf{(f)}}
%		\psfrag{G}[r][]{\textbf{(g)}}
%		\psfrag{H}[r][]{\textbf{(h)}}
%    \psfrag{error}[c][]{\NMSE}
%    \psfrag{gain alpha}[c][]{gain $\alpha$}
%    \psfrag{weight w}[c][]{weight $w$}
%    \psfrag{sample length}[c][]{sample length $|S|$}
%    \psfrag{WRW sample length}[c][]{WRW sample length $|S|$}
%    \includegraphics[width=0.90\textwidth]{figs/simulation_results.eps}
%\caption{RW and WRW under highly clustered categories (top) and not clustered categories (bottom).}
%\label{fig:simulation_results}
%\vspace{-10pt}
%\end{center}
%\end{figure*}
%
%
%
%\textbf{Discussion.} 
%\heur sets the edge weights trying to achieve roughly $\w^\WIS(C_i)$ as the main goal.
%Through two natural and easy-to-interpret parameters, $\tilde{f}_\ominus$ and $\gamma$, we slightly shape $\w^\WIS(C_i)$
%to avoid black holes and improve mixing.
%The final category weights are also affected by our choice of the ``conflict resolution'' method.
%Note that a reasonable setting of these parameters (\ie $\tilde{f}_\ominus>0$ and $1<\gamma<\infty$, and any conflict resolution discussed in the paper), increases the weights of large categories (including $C_\ominus$) and decreases the weight of small categories, compared to $\w^\WIS(C_i)$.
%This makes \heur allocate category weights between the two extremes: RW 
%%(which is very inefficient but utilizes all nodes on the graph) 
%and WIS. 
%%(which is optimal in terms of estimation in the independence sampling case, but may be inefficient in practice due to poor Markov chain convergence). 
%Consequently, \heur can be considered \emph{conservative} (with respect to WIS). 
%%Since \heur cannot do worse than RW, which is \emph{conservative}.
%%\note{We can probably show it rigorously for `arithmetic'}
%
%It is also important to note that the estimation error of~$\lowhat{\vol}(C)$ or the suboptimal choice of weights do not introduce bias into the final estimate so long as convergence is attained.
%Indeed, WRW (re-weighted at the end as in Section \ref{subsec:Correcting for the bias in RW, WRW and WIS}) is by construction an unbiased estimator.
%Suboptimal weights can increase Markov chain mixing time, and/or the variance of the resulting estimator. 
%%; however, in contexts for which $\w^\WIS$ is far from $deg(v)$, even crude approximations to the optimal weights are likely to outperform (re-weighted) RW.
%However, our simulations and empirical experiments on Facebook (see Sec.~5 and~6) show that \heur is very robust and performs well even under crude approximations to the optimal weights.









\newpage
\subsection{Our practical solution: \heur}\label{subsec:heur}
\maciej{I propose to split it into 5 steps, as below.}

%A practical weight setting algorithm should trade between the amount of required input data, its accuracy, and the cost of obtaining it.
%In this section, we introduce our practical heuristic solution - {\em Stratified Weighted Random Walk} or \heur.
%\heur follows the steps and rationale of the general approach in Section \ref{sec:approach-overview} and makes the following specific choices.
%\heur uses as input only the estimates $\lowhat{\vol}(C)$ of the category volumes (see Appendix B). 
%\heur uses two natural and easy-to-interpret parameters, $\tilde{f}_\ominus$ and $\gamma$, in order to achieve approximately  $\w^\WIS(C_i)$.

%Given our estimation problem, we set the expected number of samples per category or, equivalently, the category node weight $\w^\WIS(C_i)$.
%\heur sets the edge weights trying to achieve roughly $\w^\WIS(C_i)$ as described below. 


As the main guideline, \heur tries to achieve the category weights $\w^\WIS(C_i)$ that are optimal under WIS. 
Usually, there are many edge weight settings in~$G$ that achieve~$\w^\WIS(C_i)$. 
%We choose to divide the total weight of a category equally across all $\vol(C_i)$  edges that are incident to nodes in~$C_i$ (see Eq.(\ref{eq:volume})), s.t. each edge $e$ has the same weight % $w_e$:
In our implementation, we observe that~$\vol(C_i)$ counts the number of edges incident on nodes of~$C_i$. Consequently, if for every category~$C_i$ we set in~$G$ the weights of all edges incident on nodes in~$C_i$ to
\begin{equation}\label{eq:w_e(C_i)}
%	\w_e(C_i)\ =\ \frac{n^\opt_i}{\vol(C_i)},
	\w_e(C_i)\ =\ \frac{\w^\WIS(C_i)}{\vol(C_i)}.
\end{equation}
then $\w^\WIS(C_i)$ is achieved.\footnote{There exist many other edge weight assignments that lead to $\w^\WIS(C_i)$. \eqn{\ref{eq:w_e(C_i)}} has the advantage of distributing the weights evenly across all~$\vol(C_i)$ edges.}
This simple observation is central to the \heur heuristic. 

In order to apply \eqn{\ref{eq:w_e(C_i)}}, we first have to calculate or estimate its terms $\w^\WIS(C_i)$ and $\vol(C_i)$. Below, we show how to do it in Step~1 and 2, respectively. Next, in Steps~3-5, we show how to modify these terms to account for practical problems arising mainly from the underlying graph structure. 


\subsubsection{Step 1: Category Weights Optimal Under WIS}
The optimal WIS category weights~$\w^\WIS(C_i)$ in \eqn{\ref{eq:w_e(C_i)}} are calculated as shown, under various scenarios, in Sec.~\ref{sec:Node weight setting under WIS}. Recall that in many practical settings, the weights $\w^\WIS(C_i)$ are equal across all relevant categories $C_i$. 



\subsubsection{Step 2: Estimation of Category Volumes}
\maciej{This is one of the main comments - so I promoted it to a separate Step.}
The category volumes $\vol(C_i)$ in \eqn{\ref{eq:w_e(C_i)}} are, in general, unknown. 
Fortunately, it is easy and inexpensive to estimate them via short pilot runs. 
%
Indeed, in Appendix B, we derive efficient estimators of the volume ratio $\frac{\vol(C)}{\vol(V)}$. This means, that we estimate the volume $\vol(C)$ up to a constant, which is a sufficient input for \heur.
In particular, for a RW pilot run, we obtain \eqn{\ref{vol c 2 RW}}, as follows
$$
	\est{\frac{\vol(C)}{\vol(V)}}\ \ =\  \ \frac{1}{|S|}  \sum_{u\in S}\left(\frac{1}{\deg(u)}\sum_{v \in \mathcal{N}(u)}\!\! 1_{\{v\in C\}}\right).
$$
The only information required during this crawl is the category each neighbor belongs to, which is the same information as in the main run of \heur; see  Section \ref{subsec:Limited initial information}.
%$\lowhat{\vol}(C)$. 



\subsubsection{Step 3: Irrelevant Categories}
Let us group all (if any) irrelevant categories  into a single irrelevant category $C_\ominus\in \mathcal{C}$. Although $\w^\WIS(C_\ominus)=0$, Guideline 1 in Section \ref{sec:step2-general} suggests that we place some mass on irrelevant nodes to ensure convergence. In \heur, we achieve this goal by replacing $\w^\WIS(C_i)$ with
%$$
%\tilde{n}_i^\opt = \left\{
%	\begin{array}{ll}
%			n_i^\opt & \textrm{if } C_i \neq C_\ominus\\			
%			q\cdot n & \textrm{if } C_i = C_\ominus.		
%		\end{array}	
%		\right.
%$$
\begin{equation}
\tilde{\w}^\WIS(C_i) = \left\{
	\begin{array}{ll}
			\w^\WIS(C_i) & \textrm{if } C_i \neq C_\ominus\\			
			\tilde{f}_\ominus \cdot \sum_{C\neq C_\ominus} \w^\WIS(C) & \textrm{if } C_i = C_\ominus.		
		\end{array}	
		\right.
\end{equation}
The parameter $0<\tilde{f}_\ominus\ll 1$ controls the desired fraction of times we visit nodes in $C_\ominus$. The optimal choice of $\tilde{f}_\ominus$ depends on many factors, such as the distribution of relevant and irrelevant nodes on the graph and their absolute numbers. When measuring Facebook in Section~\ref{Applications}, we set~$\tilde{f}_\ominus=1\%$. %and $\tilde{f}_\ominus\rightarrow 0$ if $C_\ominus$ is relatively small.


\subsubsection{Step 4: Tiny and Unknown Categories}
Guideline 2 in Section \ref{sec:step2-general} suggests that we should avoid ``black holes''. In \heur, we achieve this goal by replacing $\vol(C_i)$ in \eqn{\ref{eq:w_e(C_i)}} with
\begin{eqnarray}
\nonumber \lowtilde{\vol}(C) &=& \max\Big\{\lowhat{\vol}(C),\ \vol_{min}\Big\},\quad \textrm{ where }\\
\nonumber \vol_{min} &=& \frac{1}{\gamma}\cdot \max_{C\neq C_\ominus}\{\lowhat{\vol}(C)\}
\end{eqnarray}
and $\lowhat{\vol}(C)\eq 0$ if $C$ is not covered by our estimate. This allows us to accommodate all unknown categories.

The parameter $\gamma\geq 1$ corresponds to the maximal magnification of our ``graph magnifying glass''. For $\gamma\eq 1$ (and constant~$\w^\WIS(C_i)$), we are back to the simple random walk. For $\gamma\rightarrow\infty$, we may face the problem of ``black holes'' as discussed in Sec.~\ref{sec:step2-general}. We recommend setting $\gamma$ to a value a few times larger than the average node degree $\bar{k}$.
%\footnote{$\bar{k}$ is often known, or can be easily estimated in the pilot RW}
In Section~\ref{Applications}, we use roughly $\gamma = 10\cdot \bar{k}$. %\note{motivate this better?}
%CTB: What about the approximate escape time rationale?


\subsubsection{Step 5: Edge Conflict Resolution}

With the above modifications, our target edge weights defined in Eq.(\ref{eq:w_e(C_i)}) can be rewritten as
%Similarly to Eq.(\ref{eq:w_e(C_i)}), we distribute the total weight of a category $C_i$ equally across all the $\vol(C_i)$  edges that are incident to nodes in $C_i$:
%Furthermore, recall that $\vol(C_i)$ counts the number of edges incident on nodes of~$C_i$. Consequently,
%if for every node category~$C_i$ we set in~$G$ the weights of all edges incident on~$C_i$ to
\begin{equation}\label{eq:tilde w_e(C_i)}
	\tilde{\w}_e(C_i)\ =\ \frac{\tilde{\w}^\WIS(C_i)}{\lowtilde{\vol}(C_i)}.
\end{equation}
%If such an assignment is possible, then WRW achieves $\tilde{\w}^\WIS(C_i)$.
%
We can directly set the weight $\w(u,v)\eq\tilde{\w}_e(C(u))\eq\tilde{\w}_e(C(v))$ of an intra-category edge $\{u,v\}$. However, for every inter-category edge, we usually have ``conflicting'' weights  $\tilde{\w}_e(C(u))\neq \tilde{\w}_e(C(v))$ required at the two ends of the edge. We choose to assign an edge weight  $\tilde{\w}_e$ that is in between these two values $\tilde{\w}_e(C(u))$ and $\tilde{\w}_e(C(v))$.
We considered several candidate  such assignments.
We may take the {\em arithmetic} or {\em geometric} mean of the conflicting weights, which we denote by $\w^{arithmetic}(u,v)$ and $\w^{geometric}(u,v)$, respectively. We may also use the {\em maximum} of the two values, $\w^{max}(u,v)$, which should improve mixing according to Guideline 3 in Section \ref{sec:step3-general}. %~\ref{subsec:Better RWR mixing through heavier external links}.
However, $\w^{max}(u,v)$ alone would also add high weight to irrelevant nodes $C_\ominus$. To avoid this undesired effect, per Guideline 1, we distinguish between the two cases by defining a hybrid solution:
$$
        \w^{hybrid}(u,v) = \left\{
        \begin{array}{ll}
                        \w^{geometric}(u,v)  & \textrm{if }C_\ominus\in\{C(u),C(v)\}\\
                        \w^{max}(u,v) &\textrm{otherwise.}
                \end{array}
                \right.
$$



This hybrid edge assignment was the one we found to work best in practice - see Section \ref{Applications}.





\subsubsection{Discussion}

%\begin{comment}
%\heur sets the edge weights trying to achieve roughly $\w^\WIS(C_i)$ as the main goal.
%Through two natural and easy-to-interpret parameters, $\tilde{f}_\ominus$ and $\gamma$, we slightly shape $\w^\WIS(C_i)$
%%%the target distribution
%to avoid black holes and improve mixing.
%It corresponds to Step~2 in Fig.~\ref{fig:diagram}. Step~3 under \heur can be decomposed into two substeps. First, we use~\eqn{\ref{eq:tilde w_e(C_i)}} to calculate the desired edge weights in~$G$. Next, we set these values to actual edges and
%%%The same objectives are taken into account when
%resolve potential conflicts.
%\end{comment}



%\noindent The above procedure has the following properties:
%\begin{itemize}
%	\item The edge weights of category $C$ are, in general, proportional to $\w'(C)/\vol(C)$, which guarantees that the resulting category weight $\w(C)$ is similar to the desired one $\w'(C)$.
%	\item The very small categories and the categories not discovered in the pilot RW are all assumed to have volume $\vol_{min}$. This is to avoid the black hole effect (see Sec.~\ref{subsec:Correlations - avoiding the black holes}), and to accommodate unknown categories.
%	\item Every inter-category edge weight is determined by the smaller (or `weightier') of the two categories. This is to improve mixing, as discussed in Sec.~\ref{subsec:Better RWR mixing through heavier external links}. Note that the larger category $C_{big}$ will receive some heavyweight edges from smaller categories, possibly resulting in $\w(C_{big})>\w'(C_{big})$. This side effect slightly shifts WRW towards RW (where $\w(C)=\vol(C)$ for every $C$), which is conservative.
%\end{itemize}




\textbf{Conservative approach.} 
\heur sets the edge weights trying to achieve roughly $\w^\WIS(C_i)$ as the main goal.
Through two natural and easy-to-interpret parameters, $\tilde{f}_\ominus$ and $\gamma$, we slightly shape $\w^\WIS(C_i)$
to avoid black holes and improve mixing.
The final category weights are also affected by our choice of the ``conflict resolution'' method.
Note that a reasonable setting of these parameters (\ie $\tilde{f}_\ominus>0$ and $1<\gamma<\infty$, and any conflict resolution discussed in the paper), increases the weights of large categories (including $C_\ominus$) and decreases the weight of small categories, compared to $\w^\WIS(C_i)$.
This makes \heur allocate category weights between the two extremes: RW 
%(which is very inefficient but utilizes all nodes on the graph) 
and WIS. 
%(which is optimal in terms of estimation in the independence sampling case, but may be inefficient in practice due to poor Markov chain convergence). 
Consequently, \heur can be considered \emph{conservative} (with respect to WIS). 
%Since \heur cannot do worse than RW, which is \emph{conservative}.
%\note{We can probably show it rigorously for `arithmetic'}


\textbf{Robustness to $\lowhat{\vol}(C)$ estimation error.} 
It is also important to note that the estimation error of~$\lowhat{\vol}(C)$ or the suboptimal choice of weights do not introduce bias into the final estimate so long as convergence is attained.
Indeed, WRW (re-weighted at the end as in Section \ref{subsec:Correcting for the bias in RW, WRW and WIS}) is by construction an unbiased estimator.
Suboptimal weights can increase Markov chain mixing time, and/or the variance of the resulting estimator. 
%; however, in contexts for which $\w^\WIS$ is far from $deg(v)$, even crude approximations to the optimal weights are likely to outperform (re-weighted) RW.
However, our simulations and empirical experiments on Facebook (see Sec.~5 and~6) show that \heur is very robust and performs well even under crude approximations to the optimal weights.


==> misc.tex <==
\section{Misc information}

\cite{Katzir2011}



\subsection{TODO}
\begin{itemize}
	\item Be consistent with $\{u,v\}$ or $(u,v)$ as undirected edges.
	\item 
	\item 
	\item 
\end{itemize}

%% Moved to 4.1.4
\subsection{Basic requirement: Know your neighbors}

In order to differentiate between the neighbors of some current node~$v$, the weighted random walk WRW must have some minimal information on these neighbors before visiting them. Based on this piece of information, WRW calculates the weights of all edges adjacent to~$v$.

Fortunately, such information is often available in most online graphs. For example, when inferring the university friendship graph (see Sec.~\ref{subsec:Friendly universities}), we use the university membership information of all~$v$'s neighbors, which, in Facebook, is available upon a single visit at~$v$.

%In another example, weighted multigraph sampling (see Sec.~\ref{subsec:Multigraph sampling}), we set the edge weight based on the relation graph this edge belongs to, which is available by construction.


Even when the relevant information is not available directly, we can still try to infer it. For example, in OSNs, we may exploit the neighbors's first and last names to find `long distance' edges that are likely to bring us to a different part of the social graph and thus improve the mixing time.
Indeed, an edge `Abdul~$\rightarrow$~John' is more likely to escape a local community than `Abdul~$\rightarrow$~Muhammad'.
%Indeed, an edge `Minas (a Greek name)~$\rightarrow$~Maciej (Polish)' is more likely to escape a `Greek clique' than `Minas~$\rightarrow$~Athina (Greek too)'.


Even mere node IDs (which are available in every crawlable system), may be exploited to set the weights.
%This is because user IDs are usually not assigned completely at random.
For example, in Facebook, user IDs used to be assigned in increasing order, which results in strong correlations between IDs and node degrees (the smaller the ID the higher the degree).
% see~\cite{Gjoka09_Facebook_arxiv}
Also, often some chunks of ID space are associated with particular servers, creating a clear correlation between ID and its geographical location.





\subsection{Applications}

There are many ways in which we can improve the accuracy of our estimation. We discuss them below.

\paragraph{Magnifying glass}
The first application is to visit more often the relevant parts of the graph, and to avoid the less relevant parts. This general technique comes in many flavors, depending on what we are trying to measure. In some cases, the samples of some node category~$C$ are completely useless and we want to avoid them as much as possible (see e.g., white nodes in Fig.~\ref{fig:illustration_magnifying_glass}). In other cases, nodes of all categories are required, but some are more valuable than others (as black nodes compared with red and yellow in Fig.~\ref{fig:illustration_magnifying_glass}).
% We illustrate this idea in Fig.~\ref{fig:illustration_magnifying_glass}.



%Potential scenarios include:
%\begin{itemize}
%	\item The nodes of interest are rare, but scattered in the graph (e.g., 'Adam' in Facebook)
%  \item The nodes of interest are rare, and form a tight community (e.g., UC Irvine). This case will be more difficult (black hole effect)
%  \item The nodes are plenty but we want to sample them even better (e.g., low degree nodes). This case might be very difficult to set the weights.
%%  \item Boost some particular edges (to improve mixing, or reduce cost)
%\end{itemize}



\paragraph{Better mixing}
We can follow more likely the shortcut edges that bring us to very different sections of the graph, which should improve mixing.
 This is exactly what they did in \cite{Boyd2004_mixing} with full knowledge of the graph.

\paragraph{Smaller costs}
When some links or nodes are more expensive then others. E.g., a high degree node can be expensive to visit, as we might have to list all its friens (see Facebook).


%\subsubsection{Multigraph support}
%A combination of the above three applications in the context of multigraph sampling \cite{Gjoka2010a}.




\subsection{Alternative approaches}
\maciej{Relate it to Focused sampling}
There are other approaches that may come to mind as alternatives to WRW.

One approach is to run RW (of a pre-specified length) within each node category separately. In a sense, this is an exploration version of stratified sampling.
There are three problems with this approach. First, we need a seed node in each category. Second, the categories must form densely connected communities; otherwise our short RW will not lose dependence on the seed nor converge. In an extreme (but rather likely) case the category may induce disconnected components. Third, with this approach we are not able to estimate the category size.

Another approach could be to perform RW on the entire graph, and for every visited node~$u$ sample with probability 1 every relevant neighbor $v$ of $u$. 
\maciej{this is analogous to Focused Sampling in WWW}
Although now the underlying RW does not suffer from lack of convergence, this approach is problematic too.
First, the number of nodes we collect from category~$C_i$ will be proportional to the size~$|C_i|$ of this category, which is usually inefficient (as in the basic RW).
Second, it is not obvious how to unbias the sample (we would probably need the node degrees of all neighbors of $v$, not only of $u$ and $v$). Third, the collected nodes have a tendency to be clustered (and thus strongly correlated); indeed, the friend of my friend is likely to be my friend too.





==> notation.tex <==

%\begin{table}
%	\centering
%		\begin{tabular}{ l | l  }
%  \hline                       
%  $G=(V,E)$ & the graph with nodes $V$ and edges $E$ \\
%  $N=|V|$ & number of nodes in $G$  \\
%  $\mathcal{C}=\{C\}, C\subset V$ & \\
%  $\deg(v)$ & degree on node $v\in V$  \\
%  $\vol(V_1)=\sum_{v\in V_1}\deg(v)$ & volume of some node set $V_1\subset V$ \\
%  $\w(v)$ & weight of node $v\in V$\\
%  $\w(u,v)$ & weight of edge $\{u,v\}\in E$\\
%  $\w(C)=\sum_{v\in C}\w(v)$ & weight of category $C\subset V$\\
%  $\w(C_1,C_2)$ & weight of every edge connecting $C_1$ and $C_2$\\
% % \w(v) & weight of node $v\in V$\\
%  \hline  
%\end{tabular}
%	\caption{Notation}
%	\label{tab:Notation}
%\end{table}


\section{Notation}
We consider an undirected graph $G=(V,E)$, with $|V|$~nodes and $|E|$~edges. 
For a node $v\in V$, denote by $\deg(v)$ its degree, and by $\mathcal{N}(v)\subset V$ the set of neighbors of~$v$. 

The graph $G$ is weighted. We denote by $\w(u,v)$ the weight of edge $\{u,v\}\in E$, and by 
\begin{equation}\label{eq:w_u}
	\w(u) = \sum_v \w(u,v)	
\end{equation}
the weight of node~$u\in V$. 

For any set of nodes $A\subseteq V$, we define its volume $\vol(A)$ and weight $\w(A)$ as
$$\vol(A) = \sum_{v\in A} \deg(v) \quad \textrm{ and } \quad \w(A) = \sum_{v\in A} \w(v),$$
respectively.

For any two sets of nodes $A\subset V$ and $B\subset V$, we denote by $E(A,B)$ the set of edges between $A$ and $B$. The sets $A$ and $B$ may overlap - we will often use $A=B$.


We collect a sample of nodes $S\subset V$, where $S$ may contain multiple copies of the same node.  

